Symmetric (Optimistic) Natural Policy Gradient for Multi-agent Learning with Parameter Convergence

Multi-agent interactions are increasingly important in the context of reinforcement learning, and the theoretical foundations of policy gradient methods have attracted surging research interest. We investigate the global convergence of natural policy gradient (NPG) algorithms in multi-agent learning. We first show that vanilla NPG may not have parameter convergence, i.e., the convergence of the vector that parameterizes the policy, even when the costs are regularized (which enabled strong convergence guarantees in the policy space in the literature). This non-convergence of parameters leads to stability issues in learning, which becomes especially relevant in the function approximation setting, where we can only operate on low-dimensional parameters, instead of the high-dimensional policy. We then propose variants of the NPG algorithm, for several standard multi-agent learning scenarios: two-player zero-sum matrix and Markov games, and multi-player monotone games, with global last-iterate parameter convergence guarantees. We also generalize the results to certain function approximation settings. Note that in our algorithms, the agents take symmetric roles. Our results might also be of independent interest for solving nonconvex-nonconcave minimax optimization problems with certain structures. Simulations are also provided to corroborate our theoretical findings.

==> Algorithm.tex <==
\section{Algorithm}\label{sec:alg}

We now introduce the natural PG update under softmax parameterization as follows. 

\#
  \theta^{(k+1)}&=\theta^{(k)}+\frac{\eta_\theta}{1-\gamma}\cdot A_{\theta}^{\theta^{(k)},\vartheta^{(k)}}\text{~~and~~} \mu_{\theta^{(k+1)}}(a\given s)=\mu_{\theta^{(k)}}(a\given s)\frac{\exp\big[\eta_\theta A_{\theta}^{\theta^{(k)},\vartheta^{(k)}}(s,a)/(1-\gamma)\big]}{Z^{(k)}_\theta(s)},\label{equ:NPG_1}\\ 
   \vartheta^{(k+1)}&=\vartheta^{(k)}-\frac{\eta_\vartheta}{1-\gamma}\cdot A_{\vartheta}^{\theta^{(k)},\vartheta^{(k)}} \text{~~and~~} \nu_{\vartheta^{(k+1)}}(b\given s)=\nu_{\vartheta^{(k)}}(b\given s)\frac{\exp\big[-\eta_\vartheta A_{\vartheta}^{\theta^{(k)},\vartheta^{(k)}}(s,b)/(1-\gamma)\big]}{Z^{(k)}_\vartheta(s)}, \label{equ:NPG_2}                                  
\#
where $\eta_\theta,\eta_{\vartheta}\geq 0$ are stepsizes, $A_{\theta}^{\theta^{(k)},\vartheta^{(k)}}$ and $A_{\vartheta}^{\theta^{(k)},\vartheta^{(k)}}$ are advantages functions defined as
$A^{\theta,\vartheta}_{\theta}(s,a):=\sum_{b\in\cB}\nu_\vartheta(b\given s) A^{\theta,\vartheta}(s,a,b),~A^{\theta,\vartheta}_{\vartheta}(s,b):=\sum_{a\in\cA}\mu_\theta(a\given s) A^{\theta,\vartheta}(s,a,b)$,  $Z^{(k)}_\theta(s)$ and $Z^{(k)}_\vartheta(s)$ are the normalization vectors defined as
\$
Z^{(k)}_\theta(s):=\sum_{a\in\cA}\mu_{\theta^{(k)}}(a\given s){\exp\bigg[\frac{\eta_\theta A_{\theta}^{\theta^{(k)},\vartheta^{(k)}}(s,a)}{1-\gamma}\bigg]},\qquad Z^{(k)}_\vartheta(s):=\sum_{b\in\cB}\nu_{\vartheta^{(k)}}(b\given s){\exp\bigg[\frac{-\eta_\vartheta A_{\vartheta}^{\theta^{(k)},\vartheta^{(k)}}(s,b)}{1-\gamma}\bigg]}. 
\$
The advantage functions used can also be replaced by Q-value functions, too.


==> Nonlinear_Case.tex <==
%!TEX root = Main.tex

\subsection{Nonlinear Function Approximation}

\kz{so we think the ``nonlinear'' FA part is not enough for a whole section?}

In this section we discuss a more generalized version of the function approximation setting. Our goal is to solve the following problem:
\begin{align}
\label{eq:nonlinear_min_max}
\min_{\theta \in \mathbb{R}^d} \ \max_{\nu \in  \mathbb{R}^d}  \ g_{\theta} ^{\top} Q h_{\nu}
\end{align}
where:
\begin{align}
\label{eq:func_approx_general}
g_{\theta}(a) = \frac{e^{f^g_{\theta}(a)}}{ \sum_{a'} e^{f^g_{\theta}(a')} }, \qquad h_{\nu}(a) = \frac{e^{f^h_{\nu}(a)}}{ \sum_{a'} e^{f^h_{\nu}(a')} }\edit{.}
\end{align}
Here $f^g$ and $f^h$ are function\edit{s} which are parametrized by $\theta$ and $\nu$ respectively. Note that if the functions $f^g$ and $f^h$ are linear in the parameters, we reduce to the function approximation setting discussed so far. In particular, if we have $f^g_{\theta}(a) = \theta(a)$ and $f^h_{\nu}(a) = \nu(a)$ we are back to the case of tabular softmax.

%\kz{KZ stopped here..}
From the analysis for linear function approximation, the approach that we take to solving such a problem is to convert this to an equivalent problem in the space of action vectors (which are probabilities), regularize the objective with the entropy, and solve this new regularized problem, i.e., find the QRE. For simplicity of presentation, we assume that the functions $f^g$ and $f^h$ are the same and denote it by $f$. The reformulation and regularization lead to the following problem:

\begin{align}
\label{eq:func_approx_super}
\min_{g_{\theta} \in \Delta '} \ \max_{h_{\nu}  \in \Delta ' }  \ g_{\theta} ^{\top} Q h_{\nu} - \tau \mathcal{H}(g_{\theta}) + \tau \mathcal{H}(h_{\nu}) 
\end{align}
where $\Delta' \subset \Delta$ is a subset of the simplex (Recall that in the case of linear function approximation, we had $\Delta ' = \tilde{\Delta}$ defined in Equation \eqref{eq:Delta_tilde_def}). This comprises of all distributions which can be represented by the function approximation in Equation \eqref{eq:func_approx_general}. We have the following proposition which provides a characterization for the set $\Delta'$ to be convex and thereby making the problem \eqref{eq:func_approx_super} `easy' to solve:\kz{I seem to be not able to find the proof for this theorem}
\begin{proposition}
\label{thm:poly_conv_nonlinear}
Consider the two properties: 
\vspace{-3.5mm}
\begin{itemize}
\item $ \forall \pi \in \Delta', \ \ \exists \theta$ such that $\pi(a) =  e^{f_{\theta}(a)} \ \forall$ actions $a$. 
\item  $\exists \theta \text{ such that } f_\theta = \log  \left( \lambda e^{f_{\theta_1}} + (1-\lambda) e^{f_{\theta_2}}  \right)$ for all $\lambda \in (0, 1), \forall \theta_1, \theta_2 \in \mathbb{R}^d $. 
%\item The function $f_\theta$ is invertible \kz{we might need to be a bit careful here, when talking about invertibility, which ``domain'' and ``co-domain'' are we talking about for $f_\theta$? should it be $f_\theta:\RR^d\to \Delta'$?} in polynomial time, i.e., given $\pi \in \Delta'$, we can find $\theta(\pi) \in \mathbb{R}^d$ such that $\pi(a) = e^{f_{\theta(\pi)}(a)}$ for all actions $a$. \kz{Maybe we dont need the ``polynomial time part''? It sounds a bit weird since we are not considering a complexity result. I think the essential property we need is ``$f_\theta:\RR^d\to \Delta'$ is surjective''? we dont need bijective, right?} 
\end{itemize}
\vspace{-3.5mm}
If the function $f_{\theta}$ satisfies these two properties, then the Problem \eqref{eq:nonlinear_min_max} under the parametrization \eqref{eq:func_approx_general} can be solved in polynomial time. \kz{by which algorithm? can we say anything about the rate (I believe anything would be fine :))?}\kz{the current theorem sounds a bit too vague, and may be attacked.}
\end{proposition}
Note that this is not an exact characterization for the solvability of Problem \eqref{eq:nonlinear_min_max}. In fact, the first property mentioned in Proposition \ref{thm:poly_conv_nonlinear} is merely for the easy of computation and can be done without.

Note that if the function $f$ is of the following form:
\begin{align}
f = [f_1 \ f_2 \ f_3 \ \cdots f_d \ 0 \ 0 \ 0]
\end{align}
where $[f_1 f_2 f_3 \cdots f_d]: \mathbb{R}^d \rightarrow \mathbb{R}^d$ is an invertible function, we have that the set $\Delta '$ corresponding to this $f$ is in fact $\tilde{\Delta}$ defined in Equation \eqref{eq:Delta_tilde_def}. For example, consider the function:
\begin{align}
f(\theta) = [\theta(1)^3, \theta(2)^3, \cdots, \theta(d)^3, 0, 0, \cdots, 0].
\end{align}
The set of distributions covered by it is exactly equal to the set $\tilde{\Delta}$ defined in Equation \eqref{eq:Delta_tilde_def}.

\kz{can we elaborate more on the possible ``nonlinearity'' in the function class? can we give some examples that satisfies our 3 assumptions (but at least ``look'' non-trivial :))?}



\kz{echoing ur point today, I think it would be super-cool to have some illustrative simulation showing that with nonlinear FA, other methods fail, and our method survive.}


















==> Proof.tex <==
\section{Convergence}\label{sec:proof}


Now we analyze the convergence of the NPG update in \S\ref{sec:alg}. The ideal goal is to show the convergence of the \emph{\textbf{duality gap}} $V^{*,\vartheta^{(k)}}(\rho)-V^{\theta^{(k)},*}(\rho)$ (either the last-iterate or the time-average one). A weaker convergence criterion can be the distance to the NE value, i.e., $\|V^{*}(\rho)-V^{\theta^{(k)},\vartheta^{(k)}}(\rho)\|$. Two ways to decompose the errors: 
\$
V^{*,\vartheta^{(k)}}(\rho)-V^{\theta^{(k)},*}(\rho)&=\underbrace{V^{*,\vartheta^{(k)}}(\rho)-V^{\theta^{(k)},\vartheta^{(k)}}(\rho)}_{\text{Gap}_{+}^{(k)}}+\underbrace{V^{\theta^{(k)},\vartheta^{(k)}}(\rho)-V^{\theta^{(k)},*}(\rho)}_{\text{Gap}_{-}^{(k)}}\\
&=\underbrace{V^{*,\vartheta^{(k)}}(\rho)-V^{*}(\rho)}_{\text{Gap}_{*,+}^{(k)}}+\underbrace{V^{*}(\rho)-V^{\theta^{(k)},*}(\rho)}_{\text{Gap}_{*,-}^{(k)}},
\$
where $\text{Gap}_{+}^{(k)}$ is the actual regret incurred at stage $k$, with the opponent's policy being the current one $\nu^{\vartheta^{(k)}}$ (as in online learning for matrix games); while $\text{Gap}_{+,*}^{(k)}$ is instead the gap to the actual NE value at stage $k$. 


For $\text{Gap}_{-}^{(k)}$,  by performance difference lemma 
\#
V^{\theta^{(k)},\vartheta^{(k)}}(\rho)-V^{\theta^{(k)},*}(\rho)&=\frac{1}{1-\gamma}\EE_{s\sim d_{\rho}^{\theta^{(k)},\vartheta^{(k)}},a\sim\mu_{\theta^{(k)}}(\cdot\given s),b\sim\nu_{\vartheta^{(k)}}(\cdot\given s)}\Big[A^{{\theta^{(k)}},*}(s,a,b)\Big]\label{equ:gap+1}\\
&=-\frac{1}{1-\gamma}\EE_{s\sim d_{\rho}^{\theta^{(k)},*},a\sim\mu_{\theta^{(k)}}(\cdot\given s),b\sim\nu_{\tilde\vartheta^{(k)}}(\cdot\given s)}\Big[A^{{\theta^{(k)}},{\vartheta^{(k)}}}(s,a,b)\Big],\label{equ:gap+2}
\#
where $\tilde\vartheta^{(k)} \in \argmin_{\vartheta}V_{\mu_{\theta^{(k)}},\nu_\vartheta}(\rho)$ is the best-response policy parameter for agent $2$.  However, both \eqref{equ:gap+1} and \eqref{equ:gap+2} involve the probability measure over $\cS$ that depends on $k$, i.e., $d_{\rho}^{\theta^{(k)},\vartheta^{(k)}}$ or $d_{\rho}^{\theta^{(k)},*}$. This makes it hard to do mirror descent analysis where a telescoping is needed. I have tried to do a change-of-measure, to make the measure common for all $k$. However, to do telescope, this would require a  stepsize choice depending on the distribution mismatch coefficients, e.g., $\|d_{\rho}^{\theta^{(k)},\vartheta^{(k)}}/d_\rho^*\|_{\infty}$. I think this might be the \emph{long-term effect} that differs from learning in matrix games. 


Instead, if we consider  $\text{Gap}_{*,-}^{(k)}$, we have 
\#
V^{*}(\rho)-V^{\theta^{(k)},*}(\rho)&=\frac{1}{1-\gamma}\EE_{s\sim d_{\rho}^{*},a\sim\mu^{*}(\cdot\given s),b\sim\nu^{*}(\cdot\given s)}\Big[A^{{\theta^{(k)}},*}(s,a,b)\Big]\label{equ:gaps+1}. 
%\\
%&=-\frac{1}{1-\gamma}\EE_{s\sim d_{\rho}^{\theta^{(k)},*},a\sim\mu_{\theta^{(k)}}(\cdot\given s),b\sim\tilde\nu_{\vartheta^{(k)}}(\cdot\given s)}\Big[A_{{\theta^{(k)}},{\vartheta^{(k)}}}(s,a,b)\Big],\label{equ:gaps+2}
\#
The measure over $\cS$ now will be common for all $k$. However, the advantage function $A^{{\theta^{(k)}},*}(s,a,b)$ in \eqref{equ:gaps+1} is not the one we use in \eqref{equ:NPG_1}-\eqref{equ:NPG_2}, which is $A^{{\theta^{(k)}},\vartheta^{(k)}}(s,a,b)$. \eqref{equ:gaps+1} further leads to 
\#\label{equ:gaps+3}
V^{*}(\rho)-V^{\theta^{(k)},*}(\rho)&=\frac{1}{1-\gamma}\EE_{s\sim d_{\rho}^{*},a\sim\mu^{*}(\cdot\given s),b\sim\nu^{*}(\cdot\given s)}\Big[Q^{{\theta^{(k)}},*}(s,a,b)\Big]-\frac{1}{1-\gamma}V^{{\theta^{(k)}},*}(d^*_{\rho})\notag\\
&\leq \frac{1}{1-\gamma}\EE_{s\sim d_{\rho}^{*},a\sim\mu^{*}(\cdot\given s),b\sim\nu^{*}(\cdot\given s)}\Big[Q^{{\theta^{(k)}},\vartheta^{(k)}}(s,a,b)\Big]-\frac{1}{1-\gamma}V^{{\theta^{(k)}},*}(d^*_{\rho}).
\#
Note that we can only upper-bound Q-value here using best-response, not the advantage. \eqref{equ:gaps+3} cannot be directly connected to the advantage-based update \eqref{equ:NPG_1}-\eqref{equ:NPG_2}. 

If we use Q-value, not advantage in \eqref{equ:NPG_1}-\eqref{equ:NPG_2}, we can have 
\#\label{equ:gaps+4}
&V^{*}(\rho)-V^{\theta^{(k)},*}(\rho)\leq \frac{1}{1-\gamma}\EE_{s\sim d_{\rho}^{*},a\sim\mu^{*}(\cdot\given s),b\sim\nu^{*}(\cdot\given s)}\Big[Q^{{\theta^{(k)}},\vartheta^{(k)}}(s,a,b)\Big]-\frac{1}{1-\gamma}V^{{\theta^{(k)}},*}(d^*_{\rho})\notag\\
&\quad\leq \frac{\|\nu^*/\nu_{\vartheta^{(k)}}\|_\infty}{1-\gamma}\cdot\EE_{s\sim d_{\rho}^{*},a\sim\mu^{*}(\cdot\given s),b\sim\nu_{\vartheta^{(k)}}(\cdot\given s)}\Big[Q^{{\theta^{(k)}},\vartheta^{(k)}}(s,a,b)\Big]-\frac{1}{1-\gamma}V^{{\theta^{(k)}},*}(d^*_{\rho})\notag\\
&\quad= \frac{\|\nu^*/\nu_{\vartheta^{(k)}}\|_\infty}{\eta_\theta}\cdot\EE_{s\sim d_{\rho}^{*},a\sim\mu^{*}(\cdot\given s)}\Bigg[\log\frac{\mu_{\theta^{(k+1)}}(a\given s)Z^{(k)}_{\theta}(s)}{\mu_{\theta^{(k)}}(a\given s)}\Bigg]-\frac{1}{1-\gamma}V^{{\theta^{(k)}},*}(d^*_{\rho})\notag\\
&\quad= \frac{\|\nu^*/\nu_{\vartheta^{(k)}}\|_\infty}{\eta_\theta}\cdot\EE_{s\sim d_{\rho}^{*}}\Bigg[\KL\big(\mu^*(\cdot\given s)||\mu_{\theta^{(k)}}(\cdot\given s)\big)-\KL\big(\mu^*(\cdot\given s)||\mu_{\theta^{(k+1)}}(\cdot\given s)\big)+\log Z^{(k)}_{\theta}(s)\Bigg] -\frac{1}{1-\gamma}V^{{\theta^{(k)}},*}(d^*_{\rho}).
\#
Note that now we can do telescoping. However, we still have a mismatch coefficient $\|\nu^*/\nu_{\vartheta^{(k)}}\|_\infty$ that depends on $k$ (though for softmax policy class, this value is always finite), which may grow with respect to $k$. Similarly for $\text{Gap}_{*,+}^{(k)}$, we have 
\#
&V^{*,\vartheta^{(k)}}(\rho)-V^{*}(\rho)\leq -\frac{1}{1-\gamma}\EE_{s\sim d_{\rho}^{*},a\sim\mu^{*}(\cdot\given s),b\sim\nu^{*}(\cdot\given s)}\Big[Q^{{\theta^{(k)}},\vartheta^{(k)}}(s,a,b)\Big]+\frac{1}{1-\gamma}V^{*,{\vartheta^{(k)}}}(d^*_{\rho}). 
%\notag\\
%&\quad\leq \frac{\|\nu^*/\nu_{\vartheta^{(k)}}\|_\infty}{1-\gamma}\cdot\EE_{s\sim d_{\rho}^{*},a\sim\mu^{*}(\cdot\given s),b\sim\nu_{\vartheta^{(k)}}(\cdot\given s)}\Big[Q^{{\theta^{(k)}},\vartheta^{(k)}}(s,a,b)\Big]-\frac{1}{1-\gamma}V^{{\theta^{(k)}},*}(d^*_{\rho})\notag\\
%&\quad= \frac{\|\nu^*/\nu_{\vartheta^{(k)}}\|_\infty}{\eta_\theta}\cdot\EE_{s\sim d_{\rho}^{*},a\sim\mu^{*}(\cdot\given s)}\Bigg[\log\frac{\mu_{\theta^{(k+1)}}(a\given s)Z^{(k)}_{\theta}(s)}{\mu_{\theta^{(k)}}(a\given s)}\Bigg]-\frac{1}{1-\gamma}V^{{\theta^{(k)}},*}(d^*_{\rho})\notag\\
%&\quad= \frac{\|\nu^*/\nu_{\vartheta^{(k)}}\|_\infty}{\eta_\theta}\cdot\EE_{s\sim d_{\rho}^{*}}\Bigg[\KL\big(\mu^*(\cdot\given s)||\mu_{\theta^{(k)}}(\cdot\given s)\big)-\KL\big(\mu^*(\cdot\given s)||\mu_{\theta^{(k+1)}}(\cdot\given s)\big)+\log Z^{(k)}_{\theta}(s)\Bigg] -\frac{1}{1-\gamma}V^{{\theta^{(k)}},*}(d^*_{\rho}).
\#
However, as now we have $-Q$ non-positive, we cannot use the mismatch coefficient as in \eqref{equ:gaps+4}. 

\paragraph{Other thoughts:}
\begin{itemize}
%	\item Can we use $A^{{\theta^{(k)}},*}(s,a,b)$ and $A^{*,{\vartheta^{(k)}}}(s,a,b)$ in the update \eqref{equ:NPG_1}-\eqref{equ:NPG_2}, as the \emph{worst-case} counterfactual advantage? If so, the mirror descent analysis might go through, starting from \eqref{equ:gaps+1} directly. However, we may still need a change of measure $\|\nu^*/\|_\infty$. Also, in \emph{sample-based} version, how to obtain an estimate of this worst-case counterfactual? 
	\item Is there any other way of  decomposing the duality gap?
	\item If not, will choosing different stepsizes for two players $\eta_\theta$ and $\eta_\vartheta$ help? Have tried, but seems not obvious, as unlike the recent nonconvex-nonconcave minimax optimization results, it seems that no smoothness constant is used in this type of analysis, to guide the choice of stepsizes.  
	\item Compared to MWU solving zero-sum matrix games,  the key subtlety here in Markov games is that the opponent's policy enters the update \eqref{equ:NPG_1}-\eqref{equ:NPG_2} not only via a probability measure  over its actions on the payoff matrix $[A^{\theta,\vartheta}(s,a,b)]_{a\in\cA,b\in\cB}$, but also via affecting the payoff matrix per se. 
%	\item  to choose, since unlike the recent nonconvex-nonconcave minimax optimization results, our analysis of NPG seems to be independent of the smoothness of the value function, which is usually the key for choosing different stepsizes in those works.  
\end{itemize}



 




==> Proof_2.tex <==
\section{Episodic Setting}

Now we take one step back, and consider the episodic setting with finite horizons. 


\subsection{Q1: Exponential dependence on $H$?}

Recall that  in the notes by Qiaomin and Yudong, i.e., Theorem 1, there is an exponential dependence on $H$, $C^H$,  even in the MDP setting where {\tt{P2}} has no effect. There are several questions need to be clarified: 

\begin{enumerate}
	\item Is it because of the algorithm? Note that in the MDP setting, Algorithm 1 is not the natural policy gradient, since in that case $Q^{\bar{\sigma}^\ell}_h\big(x,a,\nu^\ell_h(x)\big)$ in the summation  should be $Q^{{\sigma}^\ell}_h\big(x,a,\nu^\ell_h(x)\big)=Q^{{\mu}^\ell}_h\big(x,a\big)$, i.e., no average over all the policies before $\ell$. 
	\item Is it because of the analysis? In my understanding, in the proof of Theorem 1, term $T_3$ is where the trouble is. In the MDP setting, the mirror-descent-type  analysis did not yield this error. 
	\item Is it because it violates the hardness result in \cite{bai2020near}, i.e., Theorem 6  therein, regarding  finding the best-response? Though not being directly connected, the proof in the notes shows that if we can somehow make $V_1^{{\tt{br}(\bar{\nu}^K)}\times \bar{\nu}^K}(x)-V_1^{\bar{\sigma}^K}(x)\leq {\tt poly}(\cS,\cA,H,K)$, then it means that we can find a  ``best-response'' to $\bar{\nu}^K$ (by marginalizing $\bar{\nu}^K$). Note that we did not use the property that $\bar{\nu}^K$ has to be a ``Markov policy'', i.e., the current proof seems to work for any such a policy $\bar{\nu}^K$, by considering the performance of the two agents ``separately'' (using MWU-type of online learning argument). This might be where the issue is. Need more discussions on this.
\end{enumerate}

Now let's see if we can remove $C^H$ for the MDP setting, without changing the current algorithm (using $\bar{\sigma}^\ell$ instead of $\sigma^\ell$ in $Q$). Specifically, for the \textbf{Induction Step} on page 7, we  consider the following difference term for the MDP setting:
\#
&V_h^{{\tt br}(\bar{\nu}^k)\times \bar{\nu}^k}(x)-V_h^{\bar{\sigma}^k}(x)=V_h^{\mu^*}(x)-V_h^{\bar{\mu}^k}(x)\notag\\
&\qquad=\EE_{\mu^*}\bigg[V_{h+1}^{\mu^*}(x_{h+1})-V_{h+1}^{\bar{\mu}^k}(x_{h+1})\biggiven x_h=x\bigg]+\Big\la Q_h^{\bar{\mu}^k}(x,\cdot),~\mu^*_h(x)-\bar{\mu}^k_h(x)\Big\ra\notag\\
&\qquad=\EE_{\mu^*}\bigg[V_{h+1}^{\mu^*}(x_{h+1})-V_{h+1}^{\bar{\mu}^k}(x_{h+1})\biggiven x_h=x\bigg]+\frac{1}{k}\sum_{\ell\in[k]}\Big\la Q_h^{\bar{\mu}^\ell}(x,\cdot),~\mu^*_h(x)-\bar{\mu}^\ell_h(x)\Big\ra\notag\\
&\qquad\qquad+\frac{1}{k}\sum_{\ell\in[k]}\Big\la Q_h^{\bar{\mu}^k}(x,\cdot)-Q_h^{\bar{\mu}^\ell}(x,\cdot),~\mu^*_h(x)-\bar{\mu}^\ell_h(x)\Big\ra\label{equ:decomp_1}\\
&\qquad=\EE_{\mu^*}\bigg[V_{h+1}^{\mu^*}(x_{h+1})-V_{h+1}^{\bar{\mu}^k}(x_{h+1})\biggiven x_h=x\bigg]+\Big\la Q_h^{\bar{\mu}^k}(x,\cdot),~\mu^*_h(x)-{\mu}^k_h(x)\Big\ra+\Big\la Q_h^{\bar{\mu}^k}(x,\cdot),~{\mu}^k_h(x)-\bar{\mu}^k_h(x)\Big\ra,\label{equ:decomp_2}
%&\qquad=\EE_{{\tt br}(\bar{\nu}^K),\bar{\nu}^K}\bigg[V_{h+1}^{{\tt br}(\bar{\nu}^K)\times \bar{\nu}^K}(x_{h+1})-V_{h+1}^{\bar{\sigma}^K}(x_{h+1})\biggiven x_h=x\bigg]+\Big\la Q_h^{\bar{\sigma}^K}(x,\cdot,\cdot),~\big({\tt br}(\bar{\nu}^K)\big)_h(x)-\bar{\mu}^K_h(x)\Big\ra,
\#  
where $\mu^*$ is the optimal policy, i.e., the best-response w.r.t. $\bar{\nu}^k$ (note that this holds for any $k\in[K]$).  If we follow the decomposition in \eqref{equ:decomp_1},  the same issue will occur: bounding the last term in \eqref{equ:decomp_1} leads to an additional term times $\sqrt{\vartheta/k}$, yielding the same $C^H$ dependence. If we instead follow \eqref{equ:decomp_2}, and care about the performance of the ``average policy'' $\bar{\mu}^K$, then we obtain
\#
V_1^{\mu^*}(x)-V_1^{\bar{\mu}^K}(x)&=\sum_{h\in[H]}\EE_{\mu^*}\Big[\Big\la Q_h^{\bar{\mu}^K}(x,\cdot),~\mu^*_h(x)-{\mu}^K_h(x)\Big\ra+\Big\la Q_h^{\bar{\mu}^K}(x,\cdot),~{\mu}^K_h(x)-\bar{\mu}^K_h(x)\Big\ra\Big]\notag\\
&\leq {\tt Poly}(H)\cdot\cO\bigg(\frac{1}{\sqrt{K}}\bigg)+\sum_{h\in[H]}\EE_{\mu^*}\Big[\Big\la Q_h^{\bar{\mu}^K}(x,\cdot),~{\mu}^K_h(x)-\bar{\mu}^K_h(x)\Big\ra\Big],\label{equ:last_average_output}
\#
however, the last term seems to be unable to be controlled. Alternatively, one can also replace the $K$ in \eqref{equ:last_average_output} by $k$, and sum-up over $k$. However, the last term cannot be canceled out, either. 
Hence, considering the ``average policy'' $\bar{\mu}^k$ directly seems not to be a good idea. This seems to be something too good to be true, since it returns some ``last-iterate'' guarantee for $\bar{\mu}^K$. Saying something about the average policy $\bar{\mu}^K$ can be true for the bandit case (due to convexity), but not for the MDP case, since the relationship between $\frac{1}{K}\sum_{k\in[K]}{V}_1^{\mu^k}$ and ${V}_1^{\bar{\mu}^K}$ is not clear here. 


Though we cannot have guarantee for ${V}_1^{\bar{\mu}^K}$, we can have one for $\frac{1}{K}\sum_{k\in[K]}{V}_1^{\mu^k}$, by simply replacing all the term $\bar{\mu}^k$ above by $\mu^k$. This will of course also change the update-rule, from using $Q_h^{\bar{\mu}^k}$ to $Q_h^{{\mu}^k}$. This will give us 
\$
V_1^{\mu^*}(x)-\frac{1}{K}\sum_{k\in[K]}{V}_1^{\mu^k}(x)\leq {\tt Poly}(H)\cdot\cO\bigg(\frac{1}{\sqrt{K}}\bigg),
\$
a standard argument by the natural PG/mirror descent analysis. Additionally, one can show ${V}_1^{\mu^k}$ is monotonically non-decreasing, leading to a guarantee for the last-iterate policy $\mu^K$, by using 
\$
V_1^{\mu^*}(x)-{V}_1^{\mu^K}(x)\leq V_1^{\mu^*}(x)-\frac{1}{K}\sum_{k\in[K]}{V}_1^{\mu^k}(x).
\$ 

 
%\begin{algorithm}[!thpb]
%	\caption{Optimistic Natural PG: agent 1 (maximizer), full-information} 
%	\label{alg:Opt_NPG_agent_1}
%	\begin{algorithmic}[1]
%		\STATE Initialization: for all $(s,a,h)$, $\overline{V}_h(s)\leftarrow H$, $\overline{q}_h(s,a)\leftarrow 0$, $\mu_h^1(a\given s)\leftarrow 1/A$
%%		\INPUT stuff
%		\FOR{episodes $k = 1, \cdots K$}
%%		\STATE Sample state $s_1$
%		\FOR{steps $h=1,\cdots, H$}
%		\STATE for all $s\in\cS,a\in\cA$, update value functions: 
%		\$&\overline{V}^{k+1}_h(s)\leftarrow\min\big\{(1-\alpha_k)\cdot\overline{V}^{k}_h(s)+\alpha_k\cdot\DD_{\mu^k\times \nu^k}\big(r_h(s,a,b)+\PP_h \overline{V}^{k}_{h+1}\big)+\beta_h^{k},~H\big\}\\
%		&\overline{q}_h^{k+1}(s,a)\leftarrow (1-\alpha_k)\cdot\overline{q}_h^{k}(s,a)+\alpha_k \cdot\DD_{\nu^k}\big(r_h(s,a,b)+\PP_h \overline{V}^{k}_{h+1}\big)\textcolor{red}{this step may not be necessary}
%		\$ 
%		\STATE for all $s\in\cS$, update policy:
%		\$
%		\mu_h^{k+1}(\cdot\given s)\propto \exp\big[(\overline{\eta}_k/\alpha_k)\cdot\overline{q}_h^{k}(s,\cdot)\big]
%		\$
%		\ENDFOR
%		\ENDFOR
%	\end{algorithmic}
%\end{algorithm}
%
%\begin{algorithm}[!thpb]
%	\caption{Optimistic Natural PG: agent 2 (minimizer), full-information} 
%	\label{alg:Opt_NPG_agent_2}
%	\begin{algorithmic}[1]
%		\STATE Initialization: for all $(s,b,h)$, $\underline{V}_h(s)\leftarrow 0$, $\underline{q}_h(s,b)\leftarrow 0$, $\nu_h^1(b\given s)\leftarrow 1/B$
%%		\INPUT stuff
%		\FOR{episodes $k = 1, \cdots K$}
%%		\STATE Sample state $s_1$
%		\FOR{steps $h=1,\cdots, H$}
%		\STATE for all $s\in\cS,b\in\cB$, update value functions: 
%		\$&\underline{V}^{k+1}_h(s)\leftarrow\max\big\{(1-\alpha_k)\cdot\underline{V}^{k}_h(s)+\alpha_k\cdot\DD_{\mu^k\times \nu^k}\big(r_h(s,a,b)+\PP_h \underline{V}^{k}_{h+1}\big)-\beta_h^{k},~0\big\}\\
%		&\underline{q}_h^{k+1}(s,b)\leftarrow (1-\alpha_k)\cdot\underline{q}_h^{k}(s,b)+\alpha_k \cdot\DD_{\mu^k}\big(r_h(s,a,b)+\PP_h \underline{V}^{k}_{h+1}\big)
%		\$ 
%		\STATE for all $s\in\cS$, update policy:
%		\$
%		\nu_h^{k+1}(\cdot\given s)\propto \exp\big[-(\underline{\eta}_k/\alpha_k)\cdot\underline{q}_h^{k}(s,\cdot)\big] 
%		\$
%		\ENDFOR
%		\ENDFOR
%	\end{algorithmic}
%\end{algorithm} 



 
\subsection{Q2: NPG v.s. Nash-V learning?}



I have always been curious why there is no exponential dependence in the results for Nash-V learning in \cite{bai2020near}, since they are doing FTRL for all $s\in\cS$, backward in time for all $h\in[H]$. Now I think it can be connected to NPG/PPO as follows.

%, with an optimistic value estimate (so essentially can be called OPPO? I mean, even in the full-information case, knowing the opponent's instantaneous policy, reward, and transition, we need to add some bonus). 


In fact, if we do FTRL backwards in $h$, simply layer-by-layer, this should lead to an exponential in $H$ dependence, see for example Theorem 10 in the v1 of \cite{wei2020linear}. Note that there, because linear rate for the last-iterate can be achieved, this layer-by-layer update-rule does not cause too much trouble (as long as the $C$ therein is large enough). But for standard FTRL with sublinear and average (not last-iterate) convergence, this can be a trouble. But obviously, Nash-V does not suffer from this. We can connect them as follows. First, consider the update-rule in Algorithms  \ref{alg:Opt_NPG_agent_1} and \ref{alg:Opt_NPG_agent_2}, referred to as ``optimistic Natural PG'', as it follows the NPG direction with an optimistic estimate of the Q-function.  Then, we first have the following helper lemma. 
%Note that  the following results might  be improved using adaptive stepsizes. 

\issue{The result of no-regret using \emph{adaptive} stepsize is useful, however, it makes the update rule not an NPG anymore (but consistent  with Qiaomin's  notes).}

\begin{lemma}\label{lemma:ONPG_per_state}
For any $k\in[K]$, suppose ${\eta}^k_\mu=\frac{2}{H}\sqrt{\log A/k}$ and ${\eta}^k_\nu=\frac{2}{H}\sqrt{\log B/k}$, then for any $(s,h)\in\cS\times[H]$, following the update rules in Algorithms \ref{alg:Opt_NPG_agent_1}-\ref{alg:Opt_NPG_agent_2}, it holds that 
%there exists a constant $c$ such that
\$
&\max_{\mu}\sum_{i=1}^k \DD_{\mu\times \nu_h^{i-1}}\Big(r_h+\PP_h\overline{V}_{h+1}^{i-1}\Big)(s)-\sum_{i=1}^k \DD_{\mu_h^{i-1}\times \nu_h^{i-1}}\Big(r_h+\PP_h\overline{V}_{h+1}^{i-1}\Big)(s)\leq \sqrt{4(\log A) H^2 k}\\
%\textcolor{red}{c\sqrt{2H^4 A/K}}\\
&\sum_{i=1}^k \DD_{\mu_h^{i-1}\times \nu_h^{i-1}}\Big(r_h+\PP_h\underline{V}_{h+1}^{i-1}\Big)(s)-\min_{\nu}\sum_{i=1}^k  \DD_{\mu_h^{i-1}\times \nu}\Big(r_h+\PP_h\underline{V}_{h+1}^{i-1}\Big)(s)\leq \sqrt{4(\log B) H^2 k}.
%\textcolor{red}{c\sqrt{2H^4 B/K}}.
\$
\end{lemma}
\begin{proof}
	We prove the first inequality, while the second one follows similarly. Define 
	\$
	R_k^*:=\max_{\mu}\sum_{i=1}^k \DD_{\mu\times \nu_h^{i-1}}\Big(r_h+\PP_h\overline{V}_{h+1}^{i-1}\Big)(s)-\sum_{i=1}^k \DD_{\mu_h^{i-1}\times \nu_h^{i-1}}\Big(r_h+\PP_h\overline{V}_{h+1}^{i-1}\Big)(s)
	\$
	as the regret in the first $k$  steps at state $s$.   Note that at each $h\in[H]$, Algorithm \ref{alg:Opt_NPG_agent_1} is performing multiplicative weights updates w.r.t. the reward sequence
	\$
	\DD_{\nu^{i-1}_h}\big[\big(r_h+\PP_h \overline{V}^{i-1}_{h+1}\big)(s,\cdot,\cdot)\big],~~i=1,2,\cdots, k.
	\$
	Thus, standard regret analysis yields
	\$
	R_k^*\leq \sqrt{4(\log A) H^2k},
	\$
	if the stepsize is chosen as in the lemma. This completes the proof.
\end{proof}


\begin{algorithm}[!t]
	\caption{Optimistic Natural PG: agent 1 (maximizer), full-information} 
	\label{alg:Opt_NPG_agent_1}
	\begin{algorithmic}[1]
		\STATE Initialization: for all $(s,a,h)\in\cS\times\cA\times[H]$, $\overline{q}^0_h(s,a)\leftarrow 0$, $\mu_h^0(a\given s)\leftarrow 1/A$, $\overline{V}^{0}_{h}(s)\leftarrow 0$ and for all $k\in[K]$, $\overline{V}^{k-1}_{H+1}(s)\leftarrow 0$ 
%		\INPUT stuff
		\FOR{episodes $k = 1, \cdots K$}
%		\STATE Sample state $s_1$
		\FOR{steps $h=H,H-1,\cdots,1$}
		\STATE for all $s\in\cS,a\in\cA$, update value functions: 
		\$&\overline{V}^{k}_h(s)\leftarrow
%		\min\big\{
		(1-\alpha_k)\overline{V}^{k-1}_h(s)+\alpha_k\big(\DD_{\mu^{k-1}_h\times \nu^{k-1}_h}\big[\big(r_h+\PP_h \overline{V}^{k-1}_{h+1}\big)(s,\cdot,\cdot)\big]+\overline{\beta}_h^{k-1}\big)\\
%		,~H\big\}\\
		&\overline{q}_h^{k}(s,a)\leftarrow \DD_{\nu^{k-1}_h}\big[\big(r_h+\PP_h \overline{V}^{k-1}_{h+1}\big)(s,a,\cdot)\big]
		\$ 
		\STATE for all $s\in\cS$, update policy following the NPG direction:
		\$
		\mu_h^{k}(\cdot\given s)\propto \exp\bigg[{\eta}^k_\mu\cdot\sum_{i\in[k]}\overline{q}_h^{i-1}(s,\cdot)\bigg]
		\$
		\ENDFOR
		\ENDFOR
	\end{algorithmic}
\end{algorithm}

\begin{algorithm}[!t]
	\caption{Optimistic Natural PG: agent 2 (minimizer), full-information} 
	\label{alg:Opt_NPG_agent_2}
	\begin{algorithmic}[1]
		\STATE Initialization: for all $(s,b,h)\in\cS\times\cB\times[H]$, $\underline{q}^0_h(s,b)\leftarrow 0$, $\nu_h^0(b\given s)\leftarrow 1/B$, $\underline{V}^{0}_{h}(s)\leftarrow 0$ and for all $k\in[K]$, $\underline{V}^{k-1}_{H+1}(s)\leftarrow 0$ 
%		\INPUT stuff
		\FOR{episodes $k = 1, \cdots K$}
%		\STATE Sample state $s_1$
		\FOR{steps $h=H,H-1,\cdots,1$}
		\STATE for all $s\in\cS,b\in\cB$, update value functions: 
		\$&\underline{V}^{k}_h(s)		\leftarrow
%		\max\big\{
		(1-\alpha_k)\underline{V}^{k-1}_h(s)+\alpha_k\big(\DD_{\mu^{k-1}_h\times \nu^{k-1}_h}\big[\big(r_h+\PP_h \underline{V}^{k-1}_{h+1}\big)(s,\cdot,\cdot)\big]-\underline{\beta}_h^{k-1}\big)\\
%		,~0\big\}\\
		&\underline{q}_h^{k}(s,b)\leftarrow \DD_{\mu^{k-1}_h}\big[\big(r_h+\PP_h \underline{V}^{k-1}_{h+1}\big)(s,\cdot,b)\big]
		\$ 
		\STATE for all $s\in\cS$, update policy following the NPG direction:
		\$
		\nu_h^{k}(\cdot\given s)\propto \exp\bigg[-{\eta}^k_\nu\cdot\sum_{i\in[k]}\underline{q}_h^{i-1}(s,\cdot)\bigg]  
		\$
		\ENDFOR
		\ENDFOR
	\end{algorithmic}
\end{algorithm} 


Now we establish the following property of $\overline{V}$ and $\underline{V}$. 

\begin{lemma}\label{lemma:bar_V_property}
	The update rules in Algorithms \ref{alg:Opt_NPG_agent_1}-\ref{alg:Opt_NPG_agent_2} with $\alpha_k=1/k$ \issue{[KZ: this stepsize will not work. But otherwise, it will not be an NPG anymore..]} yield that
	\begin{enumerate}
		\item For all $(s,h,k)\in\cS\times[H]\times[K]$, $\underline{V}_h^k(s)\leq \overline{V}_h^k(s)$; 
%		\item also,   $(1/K)\sum_{k\in[K]}\underline{V}_h^k(s)\leq V_h^*(s)\leq (1/K)\sum_{k\in[K]}\overline{V}_h^k(s)$.
		\item Suppose we choose $\overline{\beta}_h^{k-1}=\sqrt{4(\log A)H^2/k}$ and $\underline{\beta}_h^{k-1}=\sqrt{4(\log B)H^2/k}$ for all $(h,k)\in[H]\times[K]$, then for all $s\in\cS$ 
		\$
		 \frac{1}{K}\sum_{k=1}^K\big(\overline{V}^k_1(s)-\underline{V}^k_1(s)\big)\leq \tilde\cO\bigg(\sqrt{\frac{4\log(AB)H^4}{K}}\bigg).
		\$
	\end{enumerate}
\end{lemma}
\begin{proof}
	For the first argument, we prove it by induction. For $h=H+1$, obviously it holds, for all $k\in[K]$ and $s\in\cS$. Suppose it holds for some $h+1$ (for all $k\in[K]$ and $s\in\cS$), we have that for any  fixed $(s,h,k)$, 
%	if $\DD_{\mu^{k-1}_h\times \nu^{k-1}_h}\big[\big(r_h+\PP_h \overline{V}^{k-1}_{h+1}\big)(s,\cdot,\cdot)\big]+\overline{\beta}_h^{k-1}<H$, then  
	\$
	\underline{V}_h^k(s)\leq \DD_{\mu^{k-1}_h\times \nu^{k-1}_h}\big[\big(r_h+\PP_h \underline{V}^{k-1}_{h+1}\big)(s,\cdot,\cdot)\big]\leq \DD_{\mu^{k-1}_h\times \nu^{k-1}_h}\big[\big(r_h+\PP_h \overline{V}^{k-1}_{h+1}\big)(s,\cdot,\cdot)\big]\leq \overline{V}_h^k(s),
	\$
	where the second inequality uses the hypothesis. 
%	;  
%	otherwise if $\DD_{\mu^{k-1}_h\times \nu^{k-1}_h}\big[\big(r_h+\PP_h \overline{V}^{k-1}_{h+1}\big)(s,\cdot,\cdot)\big]+\overline{\beta}_h^{k-1}\geq H$, then $\overline{V}_h^k(s)=H\geq \underline{V}_h^k(s)$ also holds. 
	\begin{comment}
	Moreover,  notice that $(1/K)\sum_{k\in[K]}\underline{V}_{H+1}^k(s)\leq V_{H+1}^*(s)\leq (1/K)\sum_{k\in[K]}\overline{V}_{H+1}^k(s)$ holds trivially. Suppose for all $s\in\cS$ 
	\$
	\frac{1}{K}\sum_{k\in[K]}\underline{V}_{h+1}^k(s)\leq V_{h+1}^*(s)\leq \frac{1}{K}\sum_{k\in[K]}\overline{V}_{h+1}^k(s)
	\$ holds for some $h$, then we have 
	\$
	V_h^*(s)&=\max_{\mu}\min_{\nu}\DD_{\mu\times\nu}\big(r_h+\PP_hV_{h+1}^*\big)(s)=\frac{1}{K}\max_{\mu}\sum_{i\in[K]}\min_{\nu}\DD_{\mu\times\nu}\big(r_h+\PP_hV_{h+1}^*\big)(s)\\
	&\leq \frac{1}{K}\max_{\mu}\sum_{i\in[K]}\DD_{\mu\times\nu^{i-1}_h}\big(r_h+\PP_hV_{h+1}^*\big)(s)\leq \frac{1}{K}\max_{\mu}\sum_{i\in[K]}\DD_{\mu\times\nu^{i-1}_h}\big(r_h+\PP_hV_{h+1}^*\big)(s),
	\$
	where the last inequality uses the hypothesis. By Lemma \ref{lemma:ONPG_per_state}, we further obtain that
	\$
	V_h^*(s)\leq \frac{1}{K}\Bigg[\sum_{i=1}^K \DD_{\mu_h^{i-1}\times \nu_h^{i-1}}\Big(r_h+\PP_h\overline{V}_{h+1}^{i-1}\Big)(s)+\sqrt{2(\log A) H^2 K}\Bigg]
	\$
	\end{comment}
	
	For the second argument,  notice that $\overline{V}^k_h$ and $\underline{V}^k_h$ can be equivalently written as 
	\#
	\overline{V}^k_h(s)=\sum_{i\in[k]}\alpha_k^i\Big[\DD_{\mu^{i-1}_h\times \nu^{i-1}_h}\big[\big(r_h+\PP_h \overline{V}^{i-1}_{h+1}\big)(s,\cdot,\cdot)\big]+\overline{\beta}_h^{i-1}\Big]\label{equ:unroll_overline_V}\\
	\underline{V}^k_h(s)=\sum_{i\in[k]}\alpha_k^i\Big[\DD_{\mu^{i-1}_h\times \nu^{i-1}_h}\big[\big(r_h+\PP_h \underline{V}^{i-1}_{h+1}\big)(s,\cdot,\cdot)\big]-\underline{\beta}_h^{i-1}\Big]\label{equ:unroll_underline_V},
	\#
	where $\alpha_{k}^i=\alpha_i\prod_{j=i+1}^k(1-\alpha_j)$. 
	Note that a similar result has also been established in Lemma 13 in \cite{bai2020near}. Also, note that if $\alpha_k=1/k$, then we have $\alpha_{k}^i=1/k$ (for all $i$). Hence, by denoting $\delta^k_h:=\max_{s\in\cS}\Big[\overline{V}^k_h(s)-\underline{V}^k_h(s)\Big]\geq 0$, we have 
	\$
	&\overline{V}^k_h(s)-\underline{V}^k_h(s)\leq \delta^k_h\\
	&\quad\leq  \sum_{i\in[k]}\alpha_k^i\Big(\DD_{\mu^{i-1}_h\times \nu^{i-1}_h}\big[\big(r_h+\PP_h \overline{V}^{i-1}_{h+1}\big)(\tilde s_h^k,\cdot,\cdot)\big]+\overline{\beta}_h^{i-1}\Big)-\sum_{i\in[k]}\alpha_k^i\Big(\DD_{\mu^{i-1}_h\times \nu^{i-1}_h}\big[\big(r_h+\PP_h \underline{V}^{i-1}_{h+1}\big)(\tilde s_h^k,\cdot,\cdot)\big]-\underline{\beta}_h^{i-1}\Big)\\
	&\quad= \frac{1}{k}\sum_{i\in[k]}\Big(\DD_{\mu^{i-1}_h\times \nu^{i-1}_h}\big[\big(\PP_h \overline{V}^{i-1}_{h+1}-\PP_h \underline{V}^{i-1}_{h+1}\big)(\tilde s_h^k,\cdot,\cdot)\big]+\overline{\beta}_h^{i-1}+\underline{\beta}_h^{i-1}\Big)\\
%	\\
%	&\qquad\qquad-\sum_{i\in[k]}\alpha_k^i\Big(\DD_{\mu^{i-1}_h\times \nu^{i-1}_h}\big[\big(r_h+\PP_h \underline{V}^{i-1}_{h+1}\big)(\tilde s_h^k,\cdot,\cdot)\big]-\underline{\beta}_h^{i-1}\Big)\Bigg]\\
	&\quad\leq  \frac{1}{k}\sum_{i\in[k]}\bigg(\delta_{h+1}^{i-1}+\overline{\beta}_h^{i-1}+\underline{\beta}_h^{i-1}\bigg)\leq \frac{1}{k}\sum_{i\in[k]}\delta_{h+1}^{i-1}+\underbrace{2\sqrt{4(\log A)H^2/k}+2\sqrt{4(\log B)H^2/k}}_{\Delta_k}
	\$
	where $\tilde s_h^k\in\argmax_{s\in\cS}\Big[\overline{V}^k_h(s)-\underline{V}^k_h(s)\Big]$, and the last lines follows the definition of $\delta_{h+1}^i$ and the choices of $\overline{\beta}_h^{i-1}$ and $\underline{\beta}_h^{i-1}$, and uses the fact that $\sum_{i\in[k]}1/\sqrt{i}\leq 2\sqrt{k}$.   Unrolling the above inequality and summing up for all $k\in[K]$ yield 
	\$
	&\sum_{k\in[K]}\delta^k_1\leq \sum_{k\in[K]}\Big(\Delta_k+\frac{1}{k}\sum_{i\in[k]}\delta_{2}^{i-1}\Big)\stackrel{(i)}{=}\sum_{k\in[K]}\Delta_k+\sum_{i\in[K]}\delta_{2}^{i-1}\sum_{k=i}^K\frac{1}{k}\stackrel{(ii)}{\leq}2K\Delta_K+\cO(\log K)\sum_{i\in[K-1]}\delta_{2}^{i}\\
%	\leq \Delta_K+\frac{1}{K}\sum_{i\in[K-1]}\Delta_i+\frac{1}{K}\sum_{i\in[K-1]}\frac{1}{i}\sum_{j\in[i]}\delta_{3}^{i-1}\\
	&\quad \leq 2K\Delta_K+2K\cO(\log K)\Delta_K+\cO(\log^2 K)\sum_{i\in[K]}\delta_{3}^{i-1}\leq \cdots\leq ...,
	\$
	\issue{[KZ: sad, still an exponential in $H$ here..]}
	which completes the proof.
\end{proof}

Now let's try to find the Nash equilibrium policy. Let $\bar{\mu}^k=(1/k)\sum_{i\in[k]}\mu^{i-1}$ and $\bar{\nu}^k=(1/k)\sum_{i\in[k]}\nu^{i-1}$.  We first have the following lemma. 

\begin{lemma}\label{lemma:upper_lower_bound_V}
	For any $(s,h,k)\in\cS\times[H]\times[K]$, we have $\overline{V}_{h}^k(s)\geq V_{h}^{*,\bar{\nu}^k_{h}}(s)$ and $\underline{V}_{h}^k(s)\leq V_{h}^{\bar{\mu}^k_{h},*}(s)$. 
\end{lemma}
\begin{proof}
For $h=H+1$, it holds trivially. Suppose it holds for some $h+1$, i.e., $\overline{V}_{h+1}^k(s)\geq V_{h+1}^{*,\bar{\nu}^k_{h+1}}(s)$ for all $k\in[K]$, then
\$
\overline{V}_h^k(s)&=\frac{1}{k}\sum_{i\in[k]}\bigg[\DD_{\mu^{i-1}_h\times \nu^{i-1}_h}\big[\big(r_h+\PP_h \overline{V}^{i-1}_{h+1}\big)(s,\cdot,\cdot)\big]+\overline{\beta}_h^{i-1}\bigg]\geq \frac{1}{k}\max_{\mu}\sum_{i=1}^k \DD_{\mu\times \nu_h^{i-1}}\Big(r_h+\PP_h\overline{V}_{h+1}^{i-1}\Big)(s)\\
&\geq \max_{\mu}\sum_{i=1}^k \frac{1}{k}\DD_{\mu\times \nu_h^{i-1}}\Big(r_h+\PP_h\overline{V}_{h+1}^{*,\bar{\nu}_{h+1}^{i-1}}\Big)(s)=V_h^{*,\bar{\nu}_h^k}
\$ 
where the first equation is due to \eqref{equ:unroll_overline_V}, the first inequality uses Lemma \ref{lemma:ONPG_per_state}, and the last inequality uses the hypothesis.   Note that this holds for all $k\in[K]$. This completes the proof. 
\end{proof}

Finally, combining  Lemma \ref{lemma:bar_V_property} and Lemma \ref{lemma:upper_lower_bound_V} gives us
\$
\frac{1}{K}\sum_{k\in[K]}\Big(V_{h}^{*,\bar{\nu}^k_{h}}(s)-V_{h}^{\bar{\mu}^k_{h},*}(s)\Big)\leq \frac{1}{K}\sum_{k\in[K]}\Big(\overline{V}^k_1(s)-\underline{V}^k_1(s)\Big)\leq \tilde\cO\bigg(\sqrt{\frac{4\log(AB)H^4}{K}}\bigg). 
\$
In other words, randomly picking the average policy pair $(\bar{\mu}^k,\bar{\nu}^k)$ from $k\in[K]$ yields an approximate Nash equilibrium. 


Now I understand: the key reason why Nash-V does not suffer from the exponential dependence on $H$ is mainly due to the stepsize choice, and the ``corresponding'' specific ``loss'' used in the FTRL update. 

%However, the down-side of doing Nash-V for NPG is that, we still have to extract a ``certified policy'' eventually, in order to obtain near-equilibrium policy. 





